Hydrodynamic characterization of bubble column using Dynamical High Order Decomposition approach

Bubble columns are present in several applications, such as chemical and biochemical reactors and petrochemical and environmental engineering industries. This variety of applications is why understanding the bubble columns' dynamics is essential. This paper aims to describe a 2D bubble column system by a data-driven method to comprehend its dynamics better. We provided a set of simulations considering different superficial velocities to produce training data. With this data set, we compared two approaches: the Fast Fourier transformation (FFT) and the High-Order Dynamic Mode Decomposition (HODMD). Our results showed that FFT could not adequately describe the system as it has been done for a long time in the industry. However, with a few measurement points, HODMD can well represent and reconstruct the dynamics of this complex dispersed multiphase flow system.

==> paperbib.tex <==
@Manual{fluent12user,
  title={user guide, 2009},
  author={Fluent, Ansys},
  OPTorganization={ANSYS Inc., Canonsburg, PA},
  year={12}
}

https://www.overleaf.com/project/5f0602a25155ad000102d2df@book{Hirish_1988,
  title={Numerical {C}omputation of {I}nternal and {E}xternal {F}lows},
  author={Hirish, C.},
  year={1988},
  volume={2},
  publisher={Wiley}
}

@Article{pengrobson1976,
  title={A new two-constant equation of state},
  author={Peng, Ding-Yu and Robinson, Donald B},
  journal={Industrial \& Engineering Chemistry Fundamentals},
  volume={15},
  number={1},
  pages={59--64},
  year={1976},
  publisher={ACS Publications}
}

@article{soave1972,
  title={Equilibrium constants from a modified Redlich-Kwong equation of state},
  author={Soave, Giorgio},
  journal={Chemical engineering science},
  volume={27},
  number={6},
  pages={1197--1203},
  year={1972},
  publisher={Pergamon}
}

@article{augnier1995,
    author = {Aungier, R. H.},
    title = "{A Fast, Accurate Real Gas Equation of State for Fluid Dynamic Analysis Applications}",
    journal = {Journal of Fluids Engineering},
    volume = {117},
    number = {2},
    pages = {277-281},
    year = {1995},
    month = {06},
    abstract = "{A modified form of the Redlich-Kwong two-parameter equation of state is presented. The modified equation employs the acentric factor and the critical point compressibility factor as additional parameters to improve its accuracy and to extend its application range to include the critical point. This modified equation is as simple as the original form, yet achieves substantially better prediction accuracy, including thermodynamic parameters such as enthalpy and entropy. Results from this equation, the original equation, and three other popular modified forms are compared with gas property data for several compounds to demonstrate its improved accuracy and increased application range. Practical application limits to the other modified forms are identified to guide current users of those methods.}",
    issn = {0098-2202},
    doi = {10.1115/1.2817141},
    url = {https://doi.org/10.1115/1.2817141},
    eprint = {https://asmedigitalcollection.asme.org/fluidsengineering/article-pdf/117/2/277/5530185/277\_1.pdf},
}

@article{HELTON200323,
title = "Latin hypercube sampling and the propagation of uncertainty in analyses of complex systems",
journal = "Reliability Engineering & System Safety",
volume = "81",
number = "1",
pages = "23 - 69",
year = "2003",
issn = "0951-8320",
doi = "https://doi.org/10.1016/S0951-8320(03)00058-9",
url = "http://www.sciencedirect.com/science/article/pii/S0951832003000589",
author = "J.C. Helton and F.J. Davis",
keywords = "Aleatory uncertainty, Epistemic uncertainty, Latin hypercube sampling, Monte Carlo analysis, Random sampling, Sensitivity analysis, Uncertainty analysis",
abstract = "The following techniques for uncertainty and sensitivity analysis are briefly summarized: Monte Carlo analysis, differential analysis, response surface methodology, Fourier amplitude sensitivity test, Sobol' variance decomposition, and fast probability integration. Desirable features of Monte Carlo analysis in conjunction with Latin hypercube sampling are described in discussions of the following topics: (i) properties of random, stratified and Latin hypercube sampling, (ii) comparisons of random and Latin hypercube sampling, (iii) operations involving Latin hypercube sampling (i.e. correlation control, reweighting of samples to incorporate changed distributions, replicated sampling to test reproducibility of results), (iv) uncertainty analysis (i.e. cumulative distribution functions, complementary cumulative distribution functions, box plots), (v) sensitivity analysis (i.e. scatterplots, regression analysis, correlation analysis, rank transformations, searches for nonrandom patterns), and (vi) analyses involving stochastic (i.e. aleatory) and subjective (i.e. epistemic) uncertainty."
}


@article{CINELLA2010,
title = "Bayesian quantification of thermodynamic uncertainties in dense gas flows",
journal = "Reliability Engineering & System Safety",
volume = "134",
pages = "305 - 323",
year = "2015",
issn = "0951-8320",
doi = "https://doi.org/10.1016/j.ress.2014.08.006",
url = "http://www.sciencedirect.com/science/article/pii/S0951832014001999",
author = "X. Merle and P. Cinnella",
keywords = "Bayesian calibration, Uncertainty quantification, Dense-gas flow",
abstract = "A Bayesian inference methodology is developed for calibrating complex equations of state used in numerical fluid flow solvers. Precisely, the input parameters of three equations of state commonly used for modeling the thermodynamic behavior of the so-called dense gas flows, – i.e. flows of gases characterized by high molecular weights and complex molecules, working in thermodynamic conditions close to the liquid–vapor saturation curve – are calibrated by means of Bayesian inference from reference aerodynamic data for a dense gas flow over a wing section. Flow thermodynamic conditions are such that the gas thermodynamic behavior strongly deviates from that of a perfect gas. In the aim of assessing the proposed methodology, synthetic calibration data – specifically, wall pressure data – are generated by running the numerical solver with a more complex and accurate thermodynamic model. The statistical model used to build the likelihood function includes a model-form inadequacy term, accounting for the gap between the model output associated to the best-fit parameters and the true phenomenon. Results show that, for all of the relatively simple models under investigation, calibrations lead to informative posterior probability density distributions of the input parameters and improve the predictive distribution significantly. Nevertheless, calibrated parameters strongly differ from their expected physical values. The relationship between this behavior and model-form inadequacy is discussed."
}



@article{MendezHODMD,
title = {A new automatic, very efficient method for the analysis of flight flutter testing data},
journal = {Aerospace Science and Technology},
volume = {114},
pages = {106749},
year = {2021},
issn = {1270-9638},
doi = {https://doi.org/10.1016/j.ast.2021.106749},
url = {https://www.sciencedirect.com/science/article/pii/S1270963821002595},
author = {Carlos Mendez and Soledad {Le Clainche} and Rubén Moreno-Ramos and José M. Vega},
keywords = {Flight test, Aeroelastic modes, Flutter, Dynamic mode decomposition, Higher order dynamic mode decomposition},
abstract = {This article presents a new data processing method, based on higher order dynamic mode decomposition, to analyze actual flight test experimental data. The new methodology (i) is fast and efficient, (ii) is automatic, (iii) provides a clean spectrum in terms of the frequencies and damping rates of the flutter modes, and (iv) reconstructs the spatial distribution of the modes over the aircraft surface. The method gives useful and interesting information for predicting flutter and is suitable to analyze flight test data in real time.}
}
